Learning Search Space Partition for Black-box Optimization using Monte Carlo Tree Search

High dimensional black-box optimization has broad applications but remains a challenging problem to solve. Given a set of samples $\{\vx_i, y_i\}$, building a global model (like Bayesian Optimization (BO)) suffers from the curse of dimensionality in the high-dimensional search space, while a greedy search may lead to sub-optimality. By recursively splitting the search space into regions with high/low function values, recent works like LaNAS shows good performance in Neural Architecture Search (NAS), reducing the sample complexity empirically. In this paper, we coin LA-MCTS that extends LaNAS to other domains. Unlike previous approaches, LA-MCTS learns the partition of the search space using a few samples and their function values in an online fashion. While LaNAS uses linear partition and performs uniform sampling in each region, our LA-MCTS adopts a nonlinear decision boundary and learns a local model to pick good candidates. If the nonlinear partition function and the local model fits well with ground-truth black-box function, then good partitions and candidates can be reached with much fewer samples. LA-MCTS serves as a \emph{meta-algorithm} by using existing black-box optimizers (e.g., BO, TuRBO) as its local models, achieving strong performance in general black-box optimization and reinforcement learning benchmarks, in particular for high-dimensional problems.

==> previous_theory.tex <==
\iffalse
\section{Theoretical Foundations}
First we want to analyze Turbo, which reveals why it is suboptimal in terms of black-box approximation.

We consider optimization of a black-box function $f$ in a $d$-dimensional region $R$ of diameter $D(R)$. A naive way to do it is to use sampling: we sample $N$ points $\{\vx_i\}_{i=1}^N$ (ideally as evenly spaced as possible), get their true values $\{\vy_i\}$, build a model $\hat f$ and find the maximum $\vx^* = \arg\max_\vx \hat f(\vx)$. 
While there could be many different ways to learn a model $\hat f$ (e.g., Gaussian Processes), we assume a very simple but universal relationship between the error $\epsilon$ of the model, the sample count $N$ and the diameter $C$:
\begin{equation}
    N = \left(\frac{D(R)}{\epsilon}\right)^d
\end{equation}
where $\epsilon = \max_{\vx\in R} |f(\vx) - \hat f(\vx)|$ is the maximal error between the ground truth function $f$ and its approximate $\hat f$. This equation can be achieved by $\epsilon$-ball filling argument. 

Turning this equation around, we have:
\begin{equation}
    \epsilon = \frac{D(R)}{N^{1/d}}
\end{equation}
Intuitively, this means that the smaller the diameter, the lower the error. While increasing sample size $N$ also reduces the error, the improvement is marginal, in particular for high-dimensional space. This is the so-called ``the curse of dimensionality''. 

A natural way to design sample-efficient black-box optimization method, is to focus samples on important regions: if we could reduce $D(R)$ once in a while, we could drastically improve sample efficiency.  

\begin{theorem}[Progressive Halving]
Consider the following algorithm: in iteration $t$, we sample $N_t$ over region $R_t$, pick the best $\vx_t$ according to $\hat f_t$, build a new region $R_{t+1}$ around $x_t$ with $D_{t+1} = D(R_{t+1}) = D_t/2$, and repeat. Given $\epsilon > 0$, if we pick $N_t = (D_t / \epsilon_t)^d$ at each iteration $t$, then this algorithm achieves $\epsilon$-optimality.   
\end{theorem}
\begin{proof}
Picking $N_1$ yields an error of $\epsilon_1$. Let's compare $f(\vx_1)$ and $f(\vx^*)$, where $\vx^* \in R$ is the optimal solution in region $R$. By error bound we know that
\begin{equation}
    f(\vx^*) - \epsilon_1 \le \hat f(\vx^*) \le \hat f(\vx_1) \le f(\vx_1) + \epsilon_1 
\end{equation}
Note that $\hat f(\vx^*) \le \hat f(\vx_1)$ because $\vx_1 = \arg\max_\vx \hat f_1(\vx)$. Therefore, we know $f(\vx_1) \ge f(\vx^*) - 2\epsilon_1$. Applying the same logic for region $R_t$ and we know that 
\begin{equation}
    f(\vx_t) \ge \max_{\vx\in R_t} f(\vx) - 2\epsilon_t \ge f(\vx_{t-1}) - 2\epsilon_t \ge f(\vx^*) - 2\sum_{t'=1} \epsilon_{t'}
\end{equation}
\end{proof}

From the analysis, it is clear that the performance is critically dependent on $\epsilon_1$: if $\vx_1$ was not picked properly, then $\epsilon_1$ is large and the quality of the solution won't be very high despite follow-up refinement steps, since the algorithm is now trapped into a local optimal region. As a result, the performance won't improve, no matter how many more samples are put into that region. On the other hand, to achieve small $\epsilon$, we need $(D/\epsilon)^d$ sample complexity, which is a huge number.

One might think about a smarter approach: instead of getting stuck with one region $R_1$ after $\vx_1$ is picked, let's keep a bunch of $K$ regions and put samples to them. If $K$ is sufficiently large and include $\vx^*$, then we have the hope. 

\begin{theorem}
Same as above but we now partition $R_t$ into $2^d$ sub-regions, and pick the first $K$ according to their performance. If we assume that $\vx^*$ is always within the first $K$ regions, then with $N_t$, we achieve $\epsilon$-optimality.
\end{theorem}
\begin{proof}
Due to that assumption, we have $f(\vx_t) \ge f(\vx^*) - 2\epsilon_t$. Picking $\epsilon_t = D_1 2^{-t}$ and we know that after $T = 1 + \log_2 D_1/\epsilon$ iterations, $f(\vx_T) \ge f(\vx^*) - \epsilon$. On the other hand, the total sample $N \le \sum_t K N_t = 2^d K (1 + \log_2 D_1/\epsilon)$.
\end{proof}
Now we don't have $(1/\epsilon)^d$ anymore! However, it doesn't disappear for no reason. In fact, in the worse case, $K = (2^d)^T = (D_1/\epsilon)^d$ since we need to keep every sub-regions (and draw samples from them). However, (1) this seldom happens and (2) instead of a hard cut-off at first $K$ sub-regions, we could use a soft version (e.g., by applying multi-arm bandit (MAB) theory on these $2^d$ sub-regions) that draws more samples to good regions and fewer samples to bad regions, while keeping exploration. This leaves the opportunity for bad regions to catch up. 
\fi

\iffalse
\subsection{Picking Regions as Multi-arm Bandit}
Formally, we consider the following setting. Suppose we have $K$ regions $\{\Omega_k\}$. The global optimal $\vx^*$ resides in some unknown regions. At each iteration $t$ we visit one region $\Omega_k$, sample a data point $\vx_t \in \Omega_k$, and retrieve its value $f_t = f(\vx_t)$. Each region $\Omega_k$ has its maximal $g^*(\Omega_k) = \sup_{\vx\in\Omega_k} f(\vx)$. Getting the exact number of $g$ would require an enumeration of the region $\Omega$, which is computationally infeasible. Instead, what we have now is an estimate: $g_t(\Omega_k) = \max_{t'\le t} f(\vx_t)$. It is clear that $g_t \le g^*$, as a random variable, approaches $g^*$ when $t \rightarrow +\infty$. We could define confidence bound $r_t = r_t(\Omega_k)$ so that with high probability, the following holds: 
\begin{equation}
    g_t(\Omega_k) \ge g^*(\Omega_k) -  r_t(\Omega_k) \label{eq:lower-bound}
\end{equation}
\begin{theorem}
\label{thm:max-bound}
If $f$ is Lipschitz-continuous: $|f(\vx) - f(\vx')| \le L\|\vx-\vx'\|$ and $\vx_t$ is i.i.d sampled from region $\Omega_k$ with $f(\vx_t) \le g^*$, then with probability at least $1-\delta$, Eqn.~\ref{eq:lower-bound} holds with $r_t(\Omega_k) = \frac{L}{C}\sqrt[d]{\frac{V_k}{n_t}\ln\frac{1}{\delta}}$, where $V_k = \vol(\Omega_k)$, $n_t(\Omega_k)$ is the visitation of region $\Omega_k$ and $C$ is a norm-dependent constant.
\end{theorem}
Define the gap of each region $\Delta_k := f^* - g^*(\Omega_k)$ and $\Delta_0 := f^* - \min_\vx f(\vx)$ the maximal possible gap between two sampled function values. Now let's treat each region $\Omega_k$ as arm and apply a regret analysis similar to multi-arm bandits, we have: 
\begin{theorem}
\label{thm:regret}
Define $R_t(a_t) := f^* - g_t(\Omega_{a_t}) \ge 0$ as the regret of picking $\Omega_{a_t}$. Define the total regret $R(T) := \sum_{t=1}^T R_t(a_t)$. Then for $d > 1$, the cumulative regret $R(T) = \cO(T^{\frac{d-1}{d}}\sqrt[d]{\ln T} + K\Delta_0/T)$. 
\end{theorem}
\textbf{Remark}. Note that you can turn the regret bound of $R(T)$ into sample complexity: if there exists $T$ so that $\frac{R(T)}{T} \le \epsilon$, then there exists at least one $R_t(a_t) := f^* - g_t(\Omega_{a_t}) \le \epsilon$ which mean we already found a $\vx \in \Omega_{a_t}$ so that $f(\vx) = g_t(\Omega_{a_t}) \ge f^* - \epsilon$. To achieve that, since $R(T) \sim T^{\frac{d-1}{d}}$, $R(T)/T \sim T^{-\frac{1}{d}}$ and the sample complexity $T \sim 1/\epsilon^d$. \yuandong{Compare with regrets in other bandit papers $T^{\frac{d+1}{d+2}}$ and says that we don't consider discretization error.}
\fi
\iffalse
Note that it doesn't mean we have beaten the curse of dimensionality at all. In fact, with small $K$ and large region $\{\Omega_k\}$, it is likely that each $\Omega_k$ contains both good and bad samples, and the probability of sampling good samples are exponentially small. In this case, $c_k$ (and thus $C$) is exponentially large. The goal of arm splitting is to iteratively get rid of bad samples from $\Omega_k$ to decrease $c_k$. This causes regrets in the later stage to become much smaller and thus the cumulative regret \emph{after} multiple splitting is small. 

will be much better than $1/\epsilon^d$, if most of the bad regions (can be estimated by $\hat \Delta_{k,t} := \hat f_t^* - g_t(\Omega_k)$) do not get expanded. if $C$, the summation of all regions' $c_k$, doesn't go exponentially with $d$. That is, 
\fi

\def\good{\mathrm{good}}
\def\bad{\mathrm{bad}}

\iffalse
One central issue is how to rank exponential number of regions or arms? Traditional MAB deals with enumerable arms and the resulting algorithms scale with $\cO(K)$ where $K$ is the number of arms, which doesn't fit well with our setting. As the main contribution of this paper, we propose to recursively split  so that benefit of variance reduction overrules the cost of splitting. 
\fi
\iffalse
\subsection{Arm splitting}

Note that the upper bound of Theorem~\ref{thm:regret} is obtain by Holder's inequality. This upper bound is achieved when $n_T(\Omega_k) \propto V_k$, which is the same as we sample the entire volume $V$ uniformly, regardless of the partition. To make the regret lower, we want to get rid of bad regions which have huge volumes as soon as possible. 

$n_T(\Omega_k) \propto V_k$. 

According to the term $\sum_k c_k$ in the cumulative regret, splitting arms has a natural trade-off. More arms means more terms (each $c_k$ is positive); on the other hand, splitting one arm $k$ into 2 makes sense, if $\Omega_k$ could be split into good and bad regions ($\Omega_\good$ and $\Omega_\bad$) so that high function values are concentrated in $\Omega_\good$.

Consider the following example, suppose we have uniform distribution of function value, i.e., $U[a, b]$ in $\Omega_k$. CDF of $U[a, b]$ is a linear function $1 - (b-y) / (b-a)$ so $c_k = b - a$. Now we split the region into $\Omega_\good$ which has a distribution $U[(a+b)/2, b]$ and $\Omega_\bad$ which has a distribution $U[a, (a+b)/2]$, then $c_\good = c_\bad = c_k / 2$, $\Delta_\good = \Delta_k$ since $g(\Omega_\good) = g(\Omega_k)$, but $\Delta_\bad = \Delta_k + c_k / 2$ becomes larger. As a result, if we define $L(c_k, \Delta_k) := 6c_k\ln\frac{6c_k}{\Delta_k}$, then the overall regret is smaller:
\begin{equation}
    L(c_\good) + L(c_\bad) = 3c_k\ln\frac{3c_k}{\Delta_k} + 3c_k\ln\frac{3c_k}{\Delta_k + c_k / 2}\quad < \quad L(c_k) = 6c_k\ln\frac{6c_k}{\Delta_k}
\end{equation}

In practice, the perfect split $U[a, b] \rightarrow U[a, (a+b)/2], U[(a+b)/2, b]$ is hard to achieve. Instead, we expect $\Omega_\good$ to get rid of tails of bad samples so that $c_\good$ is reduced, and $\Omega_\bad$ to get rid of good samples so that either $\Delta_\bad$ is larger or $c_\bad$ is smaller (i.e., lower samples density around $g(\Omega_\bad)$). \yuandong{We might put a figure here.}

\begin{theorem}
If we split region $\Omega_k$ with a classifier using labels computed from K-mean, then under some conditions, $L(c_\good, \Delta_\good) + L(c_\bad, \Delta_\bad) < \gamma L(c_k, \Delta_k)$ with some $\gamma < 1$. 
\end{theorem}

\yuandong{Another effect here is that if the region is smaller, then the model built on it has higher accuracy so each sample is more likely to be close to region maximal. This also reduce $c_k$.} 
\fi

\iffalse
Picking ``actions'' that leads to good regions more frequently, leads to more samples on those good sub-regions that we never construct explicitly. Each of such partitions $\Omega$ might contain exponential number of sub-regions $\{R_j\}$ ($R_j \subseteq \Omega$), and any sample on $\Omega$ fails into one of such sub-regions with ground truth performance. Although we cannot assign distinct sampling probability over $R_j$ within $\Omega$ (we can only assign sampling probability on $\Omega$), over time each $R_j$ accumulates sufficient samples with distinctive performance. If some $R_j$ excels others, they can be further partitioned out to receive more samples.

\yuandong{Multi-arm bandits have the regret bound, which is the best we could do since it can assign different sampling probability for different arms. With recursive partition, we can only control sampling on $\Omega$ and assume this sample goes to $R_j \subseteq \Omega$ with probability proportional to $\vol(R_j)$. This will increase the regret bound in trade of exponentially less computational burden. Characterizing such a trade-off is the goal of theoretical analysis.}
\fi

% \section{Broader impact}
% Black-box optimization has a variety of applications in practice, ranging from the hyper-parameter tuning in the distributed system and database, Integrated Circuit(IC) design, Reinforcement Learning (RL), and many more. Most real-world problems are heterogeneous and high-dimensional while existing black-box solvers struggle to yield a reasonable performance in these problems. In this paper, we made our first step to show a gradient-free algorithm, for the first time, solves high-dimensional complex MuJoCo tasks, indicating its potential to other high-dimensional tasks in various domains.

% This work has the following potential positive impact on society. For example, it will improve the productivity of technology workers for the minimal cost when they want to optimize the performance of some applications. We do not foresee any negative societal consequences for this work.

\iffalse
\section{Theorems}
\subsection{Thm.~\ref{thm:max-bound}}
\begin{proof}
Let $\epsilon < 1$. Each $f_t$ is an independent random variable with cumulative density function (CDF) $F(y) = P[f_t \le y]$. By definition, $g^*$ is the upper-bound of all $f_t$ and thus $F(g^*) = 1$. We have:
\begin{equation}
    P[g_t \le y] = \prod_{t'\le t} P[f_{t'} \le y] = F^n(y)
\end{equation}
Taking $y = g^* - r_t$, we have:
\begin{equation}
    P[g_t \ge g^* - r_t] = 1 - F^n(g-r_t)
\end{equation}

Since the function is $L$-Lipschitz, we know that around the optimal solution $\vx^*_k \in \Omega_k$, the function values are also quite good:
\begin{equation}
    f(\vx) \ge f(\vx^*_k) - L|\vx-\vx^*_k| = g^* - r, \quad\forall\vx \in B\left(\vx^*_k, \frac{r}{L}\right)
\end{equation}
Since we do uniform sampling in $\Omega_k$, the probability that $\vx$ falls into a region is proportional to its volume. Therefore, we have:
\begin{equation}
    F(g-r) := P[f_t \le g-r] \le 1 - \frac{\vol(B(\vx_k^*, r/L))}{\vol(\Omega_k)} = 1 - \frac{C^d(r/L)^d}{V_k}
\end{equation}
where $C$ is a norm-dependent constant that turns $(r/L)^d$ into a ball volume. Let 
\begin{equation}
    r_t = \frac{L}{C}\sqrt[d]{\frac{V_k}{n_t}\ln\frac{1}{\epsilon}},
\end{equation}
then we have:
\begin{equation}
    P[g_t \ge g - r_t] = 1 - F^n(g-r_t) \ge 1 - \left[1 - \frac{C^d(r_t/L)^d}{V_k}\right]^n = 1 - \left(1-\frac{1}{n}\ln\frac{1}{\epsilon}\right)^n
\end{equation}
Due to the inequality that for $a < 1$ and $x > 0$, $a^x \ge 1 + x\ln a$ (which can be proven by simply showing the derivative is non-negative), if we take $a = \epsilon$ and $x = 1/n$, we have:
\begin{equation}
    \epsilon^{1/n} \ge 1 - \frac{1}{n}\ln\frac{1}{\epsilon}
\end{equation}
So we have $P[g_t \ge g - r_t] \ge 1 - \epsilon$. 
\end{proof}

\def\circle#1{{\small \textcircled{\raisebox{-0.9pt}{#1}}}}

\subsection{Thm.~\ref{thm:regret}}
\begin{proof}
Taking $\epsilon = 1 / T^3$ (and thus $\ln\frac{1}{\epsilon} = 3\ln T$) so that Eqn.~\ref{thm:max-bound} holds for all $T$ iterations and all $K$ arms with probability at least $1 - K / T^2$ by union bound, which we consider as ``good event''.

For brevity, define $g^*_k := g(\Omega_k)$ as the optimal function value within the region of $\Omega_k$ and $n_{k,t} := n_t(\Omega_k)$ the visitation count of region $\Omega_k$. Define $\Delta_k := f^* - g^*_k$ the minimal regret of each arm and $r_{k,t} := r_t(\Omega_k)$ the confidence bound. At iteration $t$, since we pick $k = a_t$ as the region to explore, it must be the case that:
\begin{equation}
    f^* + r_{k,t} \stackrel{\circle{1}}{\ge} g^*_k + r_{k,t} \stackrel{\circle{2}}{\ge} g_{k,t} + r_{k,t} \stackrel{\circle{3}}{\ge} g_{k^*,t} + r_{k^*,t} \stackrel{\circle{4}}{\ge} g^*_{k^*} = f^*
\end{equation}
where $k^*$ is the index of optimal region $\Omega_{k^*}$ where its maximum $g^*_{k^*}$ is the global optimal value $f^*$. Here \circle{1} is due to global optimality of $f^*$, \circle{2} is due to global optimality of $g^*_k$ within region $\Omega_k$: $g^*_k \ge g_{k,t}$, \circle{3} is due to the fact that we pick $a_t=k$ at iteration $t$, and \circle{4} is due to the non-negativity of confidence bound: $r_{k^*,t} \ge 0$. Therefore, since $g^*_k + r_{k,t} \ge f^*$, let $\eta := L / C$ and we have:
\begin{equation}
    \Delta_k \le r_{k,t} = \eta\sqrt[d]{\frac{V_k}{n_{k,t}}\ln\frac{1}{\epsilon}} \label{eq:bad-arm-visitation}
\end{equation}
which means that
\begin{equation}
    n_{k,t} \le \eta^d \frac{V_k}{\Delta^d_k}\ln\frac{1}{\epsilon}
\end{equation}
Intuitively, this means that for bad arm with large $\Delta_k$, its visitation count is upper-bounded. 

Now we bound the total regret. Note that for $R_t(a_t) := f^* - g_{a_t,t}$, we have:
\begin{equation}
    R_t(a_t) := f^* - g_{a_t,t} = f^* - g^*_{a_t} + g^*_{a_t} - g_{a_t,t} \le 2r_{a_t, t}
\end{equation}
due to $\Delta_{k} = f^* - g^*_{k} \le r_{k,t}$ and the property of confidence bound that $g_{k,t} \ge g^*_{k} - r_{k,t}$ with $k = a_t$. If we sum over $R_t(a_t)$ and reorganize them into $K$ arms, we get:
\begin{equation}
    R(T) \le 2\eta\sqrt[d]{\ln\frac{1}{\epsilon}} \sum_{k=1}^K \sqrt[d]{V_k} \sum_{j=1}^{n_{k,T}} j^{-1/d} 
\end{equation}
This is because for each arm $k$ we pull it $n_{k,T}$ times and each time we pay a price that is proportional to $1 / n_{k, t}$ for $n_{k,t} = 1\ldots n_{k,T}$. Assume $d > 1$ (high-dimensional case), use the bound that $\sum_{i=1}^n i^{-1/d} \le \frac{d}{d-1}n^{1-1/d}$, we know that
\begin{equation}
     R(T) \le \frac{2\eta d}{d-1}\sqrt[d]{3\ln T} \sum_{k=1}^K \sqrt[d]{V_k} n_{k,T}^{\frac{d-1}{d}}
\end{equation}
Using Holder inequality with $p = d$ and $q = \frac{d}{d-1}$, we get
\begin{equation}
     R(T) \le \frac{2\eta d}{d-1}\sqrt[d]{3\ln T} \left(\sum_{k=1}^K V_k\right)^{\frac{1}{d}}\left(\sum_{k=1}^K n_{k,T}\right)^{\frac{d-1}{d}} = \frac{2\eta d}{d-1}\sqrt[d]{3\ln T} \sqrt[d]{V} T^{\frac{d-1}{d}}
\end{equation}
where $V := \sum_k V_k$ is the total volume, a constant regardless of the partition. Therefore $R(T) = \cO(T^{\frac{d-1}{d}}\sqrt[d]{\ln T})$.

If good event doesn't happen (with prob $K / T^2$), we would pay a regret of at most $\Delta_0 := f^* - \min_\vx f(\vx)$ at each iteration $t$, yield a bound of $K\Delta_0/T$. So finally we have $R(T) = \cO(T^{\frac{d-1}{d}}\sqrt[d]{\ln T} + K\Delta_0/T)$.

\iffalse
We know that $n^{k,T} \le T$ for all arms $k$, including the optimal arm $k^*$. For those sub-optimal arms with $\Delta_k > 0$ we have $\Delta_k \le r_{k,t}$ (Eqn.~\ref{eq:bad-arm-visitation}). Therefore, we have:
\begin{equation}
R(T) \le 6\ln^2 T \sum_{k: \Delta_k\le M} c_k + 6\ln T \sum_{k: \Delta_k \ge M} c_k \left(\ln\frac{6c_k}{\Delta_k} + \ln\ln T + 1\right)
\end{equation}

\begin{equation}
R(T) \le 6\ln^2 T \sum_{k: \Delta_k\le M} c_k + 6\ln T \sum_{k: \Delta_k \ge M} c_k \left(\ln\frac{6c_k}{\Delta_k} + \ln\ln T + 1\right) + K\Delta_0/T
\end{equation}

\begin{equation}
R(T) \le 6\ln^2 T \sum_{k: \Delta_k\le M} c_k + 6\ln T \sum_{k: \Delta_k \ge M} c_k \left(\ln\frac{6c_k}{\Delta_k} + \ln\ln T + 1\right) + K\Delta_0/T
\end{equation}
\fi

\end{proof}
\fi
